Grounding Conversations with Improvised Dialogues

Effective dialogue involves grounding, the process of establishing mutual knowledge that is essential for communication between people. Modern dialogue systems are not explicitly trained to build common ground, and therefore overlook this important aspect of communication. Improvisational theater (improv) intrinsically contains a high proportion of dialogue focused on building common ground, and makes use of the yes-and principle, a strong grounding speech act, to establish coherence and an actionable objective reality. We collect a corpus of more than 26,000 yes-and turns, transcribing them from improv dialogues and extracting them from larger, but more sparsely populated movie script dialogue corpora, via a bootstrapped classifier. We fine-tune chit-chat dialogue systems with our corpus to encourage more grounded, relevant conversation and confirm these findings with human evaluations.

==> ACL 2020 Yes and/sections/data_analysis.tex <==
\section{Dataset Analysis}

In order to provide a better understanding on the characteristics of our corpus, we annotate 200 {\ya}s and 200 non-{\ya}s in {\corpus}'s development set to categorize them into specific {\ya} or non-{\ya} types. 

We classify {\ya}s into explicit {\ya}s, implicit {\ya}s, or \textit{yes-but}s. Only 15\% of all {\ya}s are explicit {\ya}s, containing phrases such as ``Yeah'' or ``Sure'' that reflects agreement. Even with such phrases, identifying explicit {\ya}s is not a trivial task because it requires semantic understanding of the relevance of the context established in the prompt and that introduced in the response. In fact, there are non-{\ya}s that contain phrases affirming agreement but have no contributions or have new contributions that lack relevance. The majority (78\%) of {\ya}s are implicit {\ya}s, meaning that the agreement is implied, often in a subtle manner. The remaining 7\% are \textit{yes-but}s. 

Non-{\ya}s are divided into \textit{contradictions} and \textit{others}. Most of the non-{\ya} were \textit{other}s, as only 5\% of candidates extracted from \corn are \textit{contradictions}, which are dialogue pairs with a response that actively negates the reality in the prompt. \textit{Other}s encompass any dialogue pairs with a response that lacks coherence to the prompt or adds no or minimal contributions.
The distribution and examples of different types of {\ya}s and non-{\ya}s are shown in Table~\ref{tab:type_distribution}. 



The main focus of our work is on {\ya}s, but we provide non-{\ya}s as part of {\corpus} for those interested in training their own classifiers. The negative samples are collected using the methods described in Section~\ref{sec:cornell}. The composition details of {\corpus} are shown in Table~\ref{tab:train_set}. 

==> ACL 2020 Yes and/sections/data_collection.tex <==
\section{Data Collection}
\label{sec:datacollection}

\begin{figure*}[h]
    \centering
    \includegraphics[width=6in]{figs/workflow_h}
    \caption{An illustration of the {\ya} collection workflow. The core {\corpus} corpus comprises {\spon} {\ya}s and \corn \xspace{\ya}s (in blue boxes). However, {\corpus} can be augmented by including other general-purpose dialogue corpora in place of \corn in this workflow, as described in Section~\ref{sec:extension}.}
    \label{fig:work-flow}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.75\paperwidth]{figs/yes-and-interface}
    \caption{Amazon Mechanical Turk interface for transcribing {\ya}s from {\spon} episodes. Approximate transcriptions with speaker turns and time stamps generated from Amazon Transcribe are provided for additional guidance.}
    \label{fig:spont_interface}
\end{figure*}

\begin{table}[h]
\begin{adjustbox}{width=\columnwidth,center}
    \centering
    \begin{tabular}{lrrrr} 
        Iteration &  1 & 2 & 3 & 4\\ \hline
        {\spon} + & 10,459 &  10,459 & 10,459 & 10,459\\
        {\spon} -- & - & - & 3,225 &5,587 \\
        \corn + & - & 3,327 & 8,464 &12,220\\
        {\corn} -- & 10,459 & 13,786 & 15,698 & 17,092\\
        Total Training Samples & 20,198 & 27,572 & 37,846 & 45,358\\ \hline
        Dev Set Acc. (Spont)& 80.9\%& 73.6\% & 71.6\% &73.0\%\\
        Dev Set Acc. (\corn) & 52.2\%& 56.8\% & 62.1\% & 64.5\%\\ \hline
        Confidence Threshold & 95\% & 70\% & 50\% & 50\% \\ 
        New Extraction Volume & 12,360 & 12,802 & 5,150 & 3,515\\  
        New Proportion of {\ya}s & 26.9\% & 44.0\% & 72.9\% & 78.4\% \\
    \end{tabular}
\end{adjustbox}
    \caption{Iterative data collection results over \corn. + indicates {\ya}s and -- indicates non-{\ya}s. These counts exclude 500 turns collected from each of \spon and \corn to form the validation set. The New Extraction Volume row indicates the new number of \ya  candidates identified with the given confidence threshold, and the New Proportion of {\ya} row show as a percentage how many of these candidates were indeed evaluated as {\ya}s by Turkers. The proportion of {\ya}s increases after each iteration despite the lower confidence threshold used to filter the new predictions with the updated classifier.}
    \label{tab:iteration-table}
\end{table}





Our data collection has five stages: 

\begin{enumerate}
    \item Manually extract {\ya}s from a rich corpus of improv to obtain an initial set of {\ya}s.\label{step:manual}
    \item Construct a \ya \textit{classifier} from the corpus of collected \ya data and negative examples.\label{step:classifier} 
    \item Use the classifier from step \ref{step:classifier} to automatically extract {\ya} candidates from a much larger but sparser dialogue corpus.\label{step:auto}
    \item If necessary, manually validate candidates before adding them to the \ya corpus. 
    \item Repeat from step~\ref{step:classifier} as needed.
\end{enumerate}

An overview of this process is shown in Figure~\ref{fig:work-flow}. 





\subsection{Core \ya Collection from {\spon}}


We select the {\spon}\footnote{\url{https://www.earwolf.com/show/spontaneanation-with-paul-f-tompkins/}} podcast as a source of concentrated {\ya}s for its relatively noise-free recording quality and high-quality volume of broad domain improv dialogue. Each episode of this podcast includes an approximately 30 minute-long improv session performed by professional improvisers. Over its 201 episodes, we identified a total of 43K lines of useful spoken dialogue.

Given the confluence of a lack of objective reality, and uninterrupted multiturn dialogue, the improvisers mostly abide by the \ya principle, and therefore {\spon} is a rich resource for natural, high-quality {\ya}s. As it exists only in audio form, and automatic transcription services are too noisy for high quality annotation use, we ask Amazon Mechanical Turk workers (Turkers) to listen to the improv sessions, view Amazon Transcribe preliminary transcriptions, and re-transcribe all of the {\ya}s that they hear using our transcription interface, shown in Figure~\ref{fig:spont_interface}. The interface is based on oTranscribe, an open-source transcription service. Although the quality of transcriptions is poor, we find that including them assists the Turkers in identifying speaker turns and also understanding parts that are sometimes incomprehensible without helping context. 

\subsubsection{Recruiting Quality Crowdworkers for Difficult Annotation Tasks}

One of the main challenges for the data collection process is to recruit competent Turkers who are able to develop a good understanding of the \ya principle.  We actively recruit potential annotators to our task by inviting denizens of the sub-Reddit TurkerNation, rather than simply inviting workers through Amazon's native task posting interface based on HIT approval rate and total number of HITs approved. Our approach enables more human-level engagement, making it easier to determine Turkers' English fluency and experience with improv. To ensure their competence, Turkers first read \ya guidelines (in the appendix) then demonstrate their level of understanding through qualification Human Intelligence Tasks (HITs), which test whether the candidates can identify if a {\ya} exists in a 30 second audio segment and transcribe it if there is one. s

Even after inviting Turkers for the actual HIT of transcribing {\ya}s, we frequently monitor the quality of the data they collect and provide feedback for incorrectly identified {\ya}s. 
Apart from base pay for each episode they work on, we provide incentives for extracting more {\ya}s. The pay for our HITs averages well above California minimum wage.
 From all of the episodes, we extract 10,959 {\ya}s, indicating about 25\% of the total number of dialogue turns in {\spon} are {\ya}s.  





\subsection{Guided Extraction from the \textit{Cornell Movie-Dialogs Corpus}}
\label{sec:cornell}


Although larger than any improv corpus, let alone \ya corpus known to date, we seek to increase our corpus volume from 10,959 turn pairs. The \textit{Cornell Movie-Dialogs Corpus} \cite[\corn]{Danescu-Niculescu-Mizil+Lee:11a} contains 304,713 turns, nearly an order of magnitude more than {{\spon}}, and it is one of the closest in domain to improv among existing dialogue datasets. However, a sample annotation of 300 randomly selected turn pairs by Turkers reveal only 11.1\% of pairs are {\ya}s. We thus use the already-collected {\ya}s to probe \corn for likely candidates, to speed the search process. Recent developments of language models pre-trained on massive text data enable the training of high-accuracy models for down-stream tasks even with a small number of samples, by leveraging the contextualized embeddings that these models learn \cite{bert,radford2019language}. We thus fine-tune an initial BERT-based sequence classifier based on the implementation of \newcite{Wolf2019HuggingFacesTS} with the {\ya}s from the {{\spon}} episodes to determine if a given dialogue pair is a {\ya}, using a high threshold (initially, a 95\% probability of being \ya) to bias for precision. We ask Turkers to validate the turn pairs identified by the classifier and add the validated pairs to our \ya corpus. This procedure can be iterated. 


For the first iteration, we train the classifier with a balanced number of non-{\ya}s chosen by random sampling from \corn, a reasonable assumption due to the relatively low concentration of {\ya}s observed. The same Turkers that extracted {\ya}s from {{\spon}} are invited to validate the {\ya} candidates filtered out by the classifier using the interface shown in Figure~\ref{fig:validation_interface}. In order to ensure consistent annotation standards among Turkers, they are given a small number of overlapping HITs against which we validated. For 90 samples of unfiltered {\ya} candidates from \corn, the two workers yield a reasonably high Cohen's $\kappa$ value of 0.74. Turkers are paid at rates consistent with their rates on the extraction-from-{{\spon}} task.


\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.75\paperwidth]{figs/validation_interface.png}
    \caption{Amazon Mechanical Turk interface for validating {\ya} candidates determined by the {\ya} classifier. Turkers are asked to correct minor errors in grammar, spelling, and punctuation for qualifying {\ya} candidates, which are then categorized as `Typo/Fix.'}
    \label{fig:validation_interface}
\end{figure*}


After the set of \corn \xspace{\ya} candidates are validated, the {\ya}s and non-{\ya}s are added to the training set to train a new classifier, and the same process is repeated. We hold out 500 dialogue pairs from each subcategory (i.e. {\spon}  {\ya}s) as the development set for monitoring the classifier's performance after each iteration. 
We incrementally lower the classification threshold for choosing a {\ya} candidate as the classifier improved. We set this threshold on each iteration except for the first by retrospective evaluation of the classifier on the actual {\ya}  candidates' labels from previous iterations. The threshold with the highest F1 score is chosen to filter new {\ya} candidates to be validated. 

We balance each progressively larger corpus with negative sample turn pairs, which are either randomly selected from \corn (round 1), selected from the rejected-but-extracted turn pairs from \corn (round 2 and later), or sampled from non-\ya turn pairs in \spon formed by random coupling of prompts and responses of the \spon \xspace{\ya}s (round 3 and later). The latter forces the classifier to make decisions based on semantic features relevant to a {\ya} instead of only stylometric features in \spon \xspace {\ya}s. We stop this iterative process after four rounds, when fewer than 5,000 new {\ya} candidates are identified by the classifier, yielding a total corpus size of 26,435 {\ya}s and 23,938 negative samples. An overview of this iterative process is summarized in Table~\ref{tab:iteration-table}. The negative sampling procedure, while somewhat ad-hoc, ultimately provides a mix of turn pairs from both corpora that is sufficient to allow extraction of {\ya}s from new corpora at high precision rates, and is sufficient for our goals. 


\begin{table*}[h!]
    \centering
\begin{adjustbox}{max width=\textwidth, center}
    \begin{tabular}{lllr} 
        \multicolumn{2}{c}{Type} & \multicolumn{1}{c}{Example} & \%  \\ \hline
        \parbox[t]{20mm}{\multirow{9}{*}{\ya}} & 
        Explicit  & 
        \makecell[l]{P: Does this map look homemade to you? \\ R: Yeah, it looks like someone without a grasp of English drew it.  }& 15\% \\ {} \\  %\cline{2-4}
        & Implicit & \makecell[l]{P: Alright, pull up that plate so I can take a picture. \\ R: Sorry, the coleslaw is definitely giving off a lot of glare. } & 78\%  \\ {} \\ %\cline{2-4}
        & \textit{yes-but} & \makecell[l]{ P: We all must say the chant that we say to the king. \\ R: No, it's too erotic, please don't.}  & 7\% \\ {}\\ 
        % & \textit{Repair} & \makecell[l]{ P: Did you see Back to the Future, where he start disappearing from the picture with his siblings? \\ R: No, it's too erotic, please don't.}  & 7\% \\ {}\\ \hline
        \parbox[t]{20mm}{\multirow{4}{*}{non-\ya}} & Contra & \makecell[l]{P: Hey, hey, aren't you afraid you'll burn out a tonsil? \\ R: Tonsil? Me? No! Me burn a tonsil?  My tonsils won't burn - As life's corners I...} & 5\% \\ {} \\ %\cline{2-4}
        & Other & \makecell[l]{P: I feel different right now. \\ R: You wait and see. You're going to marry a big hero!} & 95\% \\ %\hline 
    \end{tabular}
\end{adjustbox}
    \caption{Examples and proportions of {\ya} and non-{\ya} types from annotations of 200 {\ya}s and non-{\ya}s in \corpus's development set. Determining whether a given dialogue pair is a {\ya} or not is a non-trivial task, as the agreement or contradiction of the previous dialogue turn's context is usually implicit.}
    \label{tab:type_distribution}
\end{table*}


\subsection{Additional Notes on {\ya} Criteria}

\begin{table}
    \centering
\begin{adjustbox}{max width=\columnwidth, center}
    \begin{tabular}{lrr} 
         & {\ya}s & non-{\ya}s \\ \hline
        \spon & 10,959 & 6,087$^*$ \\
        \corn & 15,476 & 18,351 \\ \hline
        \textbf{Total} & \textbf{26,435} & \textbf{24,438} \\ \hline
    \end{tabular}
\end{adjustbox}
    \caption{Composition of {\corpus}, including the development set. {\ya}s and non-{\ya}s from \corn are validated by Turkers. $^*$\spon non-{\ya}s are sampled from random combination of prompts and responses in {\spon} {\ya}s to balance the dataset for training the classifier in the final iteration, as shown in the last column of Table~\ref{tab:iteration-table}.}
    \label{tab:train_set}
\end{table}

Although the concept of a {\ya} is easy to define and understand, there are borderline cases between a {\ya} and a non-{\ya} that make the validation phase more difficult than originally expected. One of the cases that confused Turkers in the earlier stages of data collection is the case of \textit{yes-but}s. A \textit{yes-but} is a {\ya} with a response that is coherent with the provided reality, but does not appear to provide an affirmative acceptance of a suggestion given in the prompt. These are different from \textit{contradictions} that do not align with the previously established reality. In addition, there are instances where the response is a {\ya}, but is accepted by a speaker other than the one to whom the prompt is directed. 
Some \ya responses initiates a repair of a problem encountered while accepting the prompt, due to a confusion or a possible inconsistency, by asking for clarification \cite{clark1989contributing}. While these responses may not strictly \textit{establish} more detail, they provide information for ultimately establishing new information. We elide these edge cases under the umbrella category \ya in {\corpus} as they further our top-level goal of providing relevant, actionable turn responses. Examples of some of these subtle differences are shown in Table~\ref{tab:type_distribution}.


==> ACL 2020 Yes and/sections/experiments.tex <==
\section{Experiments}

To evaluate the effect of \corpus on generating \ya responses and thus improving generated dialogue quality, we train a common architecture with a variety of fine-tuning data configurations, both with and without \corpus. Specifically, for each data configuration we fine-tune a doublehead GPT-2 model (117M-parameter version based on the implementation by \newcite{transfer-learning-conversation}), which achieved state-of-the-art performance on \persona for the ConvAI-2 dialogue competition \cite{convai}. We fine-tune the models using two learning objectives, which we weigh equally in calculating loss:

\begin{enumerate}
    \item Predicting the next word.
    \item Predicting the next correct candidate that best fits the dialogue given the dialogue history.
\end{enumerate}

The language modeling component uses pre-trained weights from OpenAI, while the candidate classification head is trained from scratch. For evaluation, we use the language modeling component of the fine-tuned model to generate single-turn responses for the {\ya} prompts in the development set. We use nucleus sampling \cite{holtzman2019curious} for the decoding step to keep only the top tokens with a cumulative probability that together exceed 0.9, from which the next token is chosen with multinomial sampling.

\subsection{Data Configurations}

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figs/ranking-interface.png}
    \caption{Interface used by human evaluators to rank responses based on their quality as a {\ya}, where a rank of 1 is most preferred. The correct ranking is shown for this example. The option ranked 1 is a \textit{yes-but}: it does not reject a reality but rather rejects a suggestion and provides refining information that is most coherent to the prompt.}
    \label{fig:ranking_interface}
\end{figure}


For our experiments, we use several established dialogue datasets as baselines, namely \persona \cite{convai}, \corn \cite{Danescu-Niculescu-Mizil+Lee:11a} (the unfiltered corpus out of which we extract {\ya}s, as described in Section~\ref{sec:cornell}), and {\dd} \cite{li-etal-2017-dailydialog}. Each of these is an English-language open-domain casual conversation corpus with 100k--300k turns. For each of these datasets, we either simply fine-tune on that dataset, or fine-tune and then further fine-tune with \corpus. In another configuration, we also fine-tune directly with \corpus on top of GPT-2. The original GPT-2 implementation prepends the personalities given in {\persona} to the dialogue sequence input before tokenization. For fine-tuning to datasets apart from {\persona}, we simply do not prepend any auxiliary information to the dialogue sequence input. 



\subsection{Human Evaluation}

Automatic metrics that rely on n-gram overlap, such as BLEU, ROUGE, and METEOR, are often used for generative models when there is little variability in the target output \cite{papineni2002bleu, lin-2004-rouge, banerjee2005meteor}. However, there can be a wide variety of responses that qualify as a good {\ya}, a problem common to open-domain generation tasks. An adequate evaluation of our models requires assessing the main {\ya} criteria: agreement with the context and the quality of the new relevant contribution, both of which are not feasible with the aforementioned metrics. Therefore, we ask human evaluators to compare the quality of the {\ya}s generated by various models and the actual response to the prompt in {\corpus} that is used as the input. 


\begin{table*}[h]
    \centering
\begin{adjustbox}{max width=\textwidth, center}
    \begin{tabular}{p{40mm}r|p{40mm}|p{90mm}}
        Dataset &  \multicolumn{1}{r}{Avg Rank $\downarrow$}  & \multicolumn{1}{l}{Example Prompt} & Example Responses \\ \Xhline{2\arrayrulewidth} \hline
        \persona& 3.67 & \multirow{5}{40mm}{\texttt{I know alotta women and I'm sure she remembers me.}} & \texttt{oh my goodness, i don't know her} \\  \cline{1-2} \cline{4-4}
        {\corpus}  & 3.41 & & \texttt{Yeah, she's a bit of a mystery.} \\  \cline{1-2} \cline{4-4}
        \multirow{2}{40mm}{{\persona}+{\corpus}} & \multirow{2}{*}{\textbf{3.17}} &  & \texttt{So you remember her? I remember her in the shower}. \\  \cline{1-2} \cline{4-4}
        Gold & 1.92 & &\texttt{She does.  From when you were a boy.} \\  \hline\hline
        \corn& 3.73 & {\multirow{6}{40mm}{\texttt{I made this beautiful salmon mousse that just looked like a puddle of spit.}}} & \texttt{What?} \\  \cline{1-2} \cline{4-4}
        {\corpus}  & 3.39 & & \texttt{And it's delicious!}\\  \cline{1-2} \cline{4-4}
        \multirow{2}{40mm}{{\corn}+{\corpus}} & \multirow{2}{*}{\textbf{3.34}} &  & \texttt{That's the kind of thing you do when you're in love.} \\  \cline{1-2} \cline{4-4}
        \multirow{2}{40mm}{Gold} & \multirow{2}{*}{2.01} & & \texttt{It was genius. It's making me hungry thinking about it.} \\ \hline\hline
        \multirow{2}{40mm}{\dd} & \multirow{2}{*}{3.37}  & \multirow{7}{40mm}{\texttt{Excuse me. Is anybody in here? I'd like a bagel. Hello? Is anybody in here?}} & \texttt{I'm sorry, sir. I'm not in the mood. I'm not in the mood.}  \\  \cline{1-2} \cline{4-4}
        \multirow{2}{40mm}{\corpus}  & \multirow{2}{*}{3.32} & &  \texttt{I'm in here. I'm just trying to make sure I can get a bagel.} \\  \cline{1-2} \cline{4-4}
        {\dd}+{\corpus} & \textbf{3.31} &  & \texttt{Oh, yeah, the guy who left the bagel.} \\  \cline{1-2} \cline{4-4}
        \multirow{2}{40mm}{Gold} & \multirow{2}{*}{1.87} & & \texttt{I can help you. The problem is that the bagels are burned.} \\ \hline\hline
    \end{tabular}
\end{adjustbox}
    \caption{Average human ranking of responses to prompts from \spon generated by models trained with {\corpus}, an existing dialog corpus, or both, based on the {\ya} criteria. Rank is scaled from 1 to 4, lower is better.}
    \label{tab:yesand-rank}
\end{table*}

 \begin{table*}[h!]
 \begin{adjustbox}{width=\textwidth,center}
     \centering
     \begin{tabular}{lll}
        Dataset  & Source & Size$^*$ \\ \hline 
        DailyDialog \cite{li-etal-2017-dailydialog} & Crowdsourced & 104K \\
        Cornell Movie-Dialogs Corpus \cite{Danescu-Niculescu-Mizil+Lee:11a} & Movie scripts &  304K \\
        Persona-chat \cite{convai} & Crowdsourced & 162K \\ 
        The Ubuntu Dialogue Corpus \cite{ubuntu} & Ubuntu chat logs & 7M \\
        Twitter Triple Conversations \cite{sordoni_context_sensitive_generation} & Social media & 6K \\
        OpenSubtitles \cite{Lison2016OpenSubtitles2016EL} & Subtitles & 441M sentences \\ 
        SubTle (Eng) \cite{ameixa2013subtitles} & Subtitles & 3.3M pairs \\ 
        London-Lund Corpus \cite{greenbaum1990london} & Various sources & 500K words \\
        London-Lund Corpus 2 \cite{poldvere2017london} & Various sources & 500K words \\ \hline
        \textbf{\corpus} ({\ya} only) & Improv, Movie scripts &  26K pairs \\ 
        \textbf{\corpus-extended} ({\ya} only) & Improv, Movie scripts, subtitles & 68K pairs \\ \hline 
     \end{tabular}
\end{adjustbox}
     \caption{A survey of publicly available English language text-based corpora frequently used for open-domain dialogue systems. The last two rows are our contribution. $^*$Size is measured as the number of total utterances (dialogue turns) unless otherwise specified.}
     \label{tab:corpora_survey}
 \end{table*}


We ask human evaluators to rank a set of four responses given a prompt, comparing the responses of a model trained only with {\corpus}, a model trained with an existing dialogue corpus, a model trained with both, and the actual response pair from the development set, denoted as ``Gold.'' These four responses are randomly ordered for each question to prevent evaluators from developing a bias for responses that frequently have a good or poor response in a set order, as shown in Figure \ref{fig:ranking_interface}. The evaluators are permitted to provide the same rank for different responses if they are equal in quality. This evaluation set contains 100 such prompts, and each is evaluated twice by different evaluators. The results of the average ranking and some of the examples generated by the models are shown in Table~\ref{tab:yesand-rank}. 



Results show that models trained only with {\corpus} or with {\corpus} and another dialogue dataset are preferred to the models trained only with another dialogue dataset, although in the case of \dd, the average ranking improves only by at most 0.06 after fine-tuning with {\corpus}. However, even the responses generated by models trained with {\corpus} are not ranked as well as the actual responses in the development set, indicating our models are still inferior to professional human improviser quality.



==> ACL 2020 Yes and/sections/intro.tex <==
\section{Introduction}

\begin{figure}[h]
    \centering
    \includegraphics[width=3in]{figs/yesand_example_accessible.png}
    \caption{Explicit (top) and implicit (bottom) examples of {\ya}s in the {\corpus} corpus. The text highlighted in \colorbox{skyblue}{light blue} reflects acceptance of the context established in the prompt (``yes'') and the text highlighted in \colorbox{orange}{orange} initiates a new relevant contribution to the dialogue (``and'').}
    \label{fig:corpus_example}
\end{figure}


For humans, dialogue is fundamentally a collaborative, cooperative process by which \textit{partners} coordinate via \textit{turns} or \textit{acts} to jointly construct a common \textit{world state} \cite{bohm2004dialogue}. Without coordination, partners may establish different or conflicting world states, leading to solipsism in the best case and conflict in the worst.   \newcite{clark1989contributing}, describe five dimensions of \textit{grounding}, by which  partners cooperate to establish \textit{common ground}, or a shared world state. The dimension of ``initiation of next relevant contribution'' is the most effective of these in expressing understanding of an ongoing dialogue, and yet is the least observed in  dialogue systems. 

\textit{Improvisational theater} (improv) is a form of theater in which most or all of what is performed is unscripted, created spontaneously by the actors in real time. Because the performance is not scripted and there is typically little to no scenery or other established environment,\footnote{except for, on occasion, external stimulus such as a suggestion from the audience} there is no objective reality that can naturally ground the scene. Hence, actors must mainly rely on dialogue in order to build a coherent scene and progressively establish a common world view. This necessitates accelerated use of the ``initiation of next relevant contribution,'' which in improv is known as the \ya principle. The \ya principle is a rule-of-thumb that suggests that a participant should accept the reality of what the other participant has said (``yes'') and expand or refine that reality with additional information (``and''). Since actors consciously abide by this principle during improv performances, there is a high proportion of these turns embedded in improv dialogue, which helps ensure scenes are coherent and interesting. 


Open-domain neural dialogue systems, by contrast, specifically lack coherence and interestingness. 
They commonly repeat previous utterances \cite{jiwei_reinforcement} or generate non-committal, generic statements such as \textit{I don't know} that are logically coherent as a response but preempt further conversation \cite{ sordoni_context_sensitive_generation, serban_hierarchical_generative_nn, li-etal-2016-diversity}.  Either of these developments leads to a conversational black hole and discourages participation in further dialogue turns. This is a critical shortcoming for open-domain dialogue agents, which, unlike task-oriented dialogue systems, are not guided by specific objectives other than entertainment \cite{challenges_in_open_domain_dialogue}. It would behoove such systems to adopt the strategies improvisers include by habit in their dialogues and, consequently, incorporating improv acts should be a key focus for the dialogue community. 




Yet, to the best of our knowledge, this has not been previously done. 
There has been work in applying improv to build believable agents that interact with humans \cite{bruce_knight_listopad_magerko_nourbakhsh_2000, winston_magerko} or generate improvised stories \cite{riedl_improv_storytelling}, but development of improv-capable systems in the neural era is largely absent, stymied, we suspect, by the lack of substantial corpora. This is unsurprising; while improv speech acts such as \ya are crucial in all dialogues, they are only highly concentrated in improv dialogues. And improv dialogues are quite difficult to collect; research collections \cite{busso2008scripted} have been far too small to be useful in the modern ML era. The art form has historically been mostly ephemeral, performed live in regional venues on shoestring budgets and rarely recorded.\footnote{The art form has long roots, extending to the Italian \textit{Commedia dell'arte} tradition from the 16th century and farces from the Roman era, but we constrain our focus to the post-20th century form developed and championed by e.g. Keith Johnstone \cite{johnstone2017impro}, Del Close \cite{halpern1994truth}, and our corpus' namesake, Viola Spolin \cite{spolin1986theater}. Spolin was the originator of \textit{Theater Games}, acting exercises that encourage the development of specific theatrical skills. As our corpus is similarly designed to elicit specific skills, we backronym it in recognition of her influence.}   Transcripts are all but absent and mainstream media products are rare.\footnote{One exception, the long-running TV show \textit{Whose Line Is It Anyway}, has, despite a large number of episodes, surprisingly little continuous improvised dialogue, due to the rapid-fire nature of the program.} However, the liberalization of high quality audio \textit{podcasts} %distribution in the form of \textit{podcasts} 
since 2014 has enabled the availability of a long tail of niche products, improv included \cite{mchugh2016podcasting}. 



Therefore we set our objective as collecting \ya-type dialogue pairs ({\ya}s) to enable their modeling by corpus-driven dialogue systems. We mine podcasts and existing movie script corpora for dialogue that abides by the \ya principle and extract
dialogue pairs from these sources to build the {\corpusfull} ({\corpus}) corpus. 
{\corpus} is a collection of more than 26,000 English dialogue turn pairs, each consisting of a \textit{prompt} and subsequent \textit{response}, which abide by the \ya principle, though in diverse manners. Examples of \ya type dialogue pairs collected for {\corpus} are in Figure~\ref{fig:corpus_example}. The corpus is substantial enough to be usable for fine-tuning existing dialogue models to encourage more \ya behavior, and beyond that may prove a valuable knowledge base for empirical sociolinguistic studies on this dialogue act.  

Our contributions are summarized as follows: 

\begin{itemize}
    \item We carefully curate {\corpusfull} ({\corpus}), the first large-scale corpus of \ya dialogue acts, sourced from improv and movie dialogues.
    \item We iteratively build a high-precision \ya classifier, which we use to mine additional {\ya}s from dialogue corpora with high volume but low \ya density. 
    \item We fine-tune existing open-domain conversational models with our corpus and confirm via human evaluations that this approach improves creative grounding. 
    \item We release our models and data for public use, including a 64,000 turn pair extension of the core \corpus, at  \url{https://justin-cho.com/spolin}.
\end{itemize}






==> ACL 2020 Yes and/sections/related_work.tex <==
\section{Related Work}

Many works have identified the same issues of repetitive or non-committal responses generated by neural conversational systems that are at least partially related to the lack of sufficiently high quality {\ya}s we deal with in this work;  approaches that mitigate these problems vary. The majority of recent works focus on diversifying the responses by modifying the training and decoding objectives \cite{li-etal-2016-diversity, jiwei_decode, li-etal-2017-adversarial, jiwei_reinforcement, xu-etal-2017-neural, shao2017}. Other methods introduce latent variables to encourage diversity \cite{serban2017hierarchical, zhao2017diversity_vae}. Some explore methods of re-weighing training instances that encourage diversity \cite{liu-etal-2018-towards-less, lison-bibauw-2017-dialogues, du-black-2019-boosting}. 

Our approach is complementary to all the model-based approaches described here, as it simply deals with the production of a particularly useful \textit{corpus}, that can be used to fine-tune on top of these methods.

We provide a survey of publicly available text-based datasets frequently used for open-domain dialogue systems and discuss their limitations for our purpose of generating grounded responses (see Table \ref{tab:corpora_survey} for an overview). 


\textit{DailyDialog} is a collection of multi-turn dialogue with manually annotated emotion and intent labels \cite{li-etal-2017-dailydialog}. \newcite{Danescu-Niculescu-Mizil+Lee:11a} created \textit{the Cornell Movie-Dialogs Corpus}, a compilation of dialogue sequences paired with meta data about the movie and characters. \persona provides dialogue sequence coupled with corresponding personas \cite{convai}. The \textit{Ubuntu Dialogue Corpus} contains 1 million dialogue turns extracted from Ubuntu chat logs, which discuss Ubuntu-related technical support \cite{ubuntu}. The \textit{Twitter Triple Corpus} is a dataset of 4K dialogue triples extracted from Twitter \cite{sordoni_context_sensitive_generation}.  \textit{OpenSubtitles} is a huge collection of subtitles that span various genres, but the absence of speaker turn annotations make it difficult to modify into dialogue format \cite{Lison2016OpenSubtitles2016EL}. \newcite{ameixa2013subtitles} use heuristics to reformat OpenSubtitles into dialogues with some limited success. \newcite{clark1989contributing} illustrate grounding in conversations with examples from the London-Lund Corpus \cite{greenbaum1990london}, a corpus of full conversations annotated with prosodic and paralinguistic features. A second version of the corpus was compiled with the same annotations standards as the first using more recent spoken and text data \cite{poldvere2017london}. 

These corpora were not collected with the criteria for {\ya}s in mind. Even for datasets with dialogue taking place in a similar domain as improv, they naturally contain only a small proportion of {\ya}s. However, the relatively large sizes of these datasets still make them useful for dialogue systems. They can be used effectively for grounded conversations if the {\ya}s or other desirable dialogue acts can be filtered out or given higher weights in training to enforce their characteristics in the responses generated. 

Our data collection approach is similar to the method of \newcite{yarowsky-1995-unsupervised}, which formalizes the bootstrapping mechanism of iteratively improving a classifier and label unlabeled data. % original Yarowsky algorithm \cite{abney2004understanding}.
% iterative data augmentation approach with a bootstrapped classifier is a variant of
% Our core \ya collection from \spont is the initial set that is used to train the base learner or ``inner loop". The resulting learner is used to label a portion of unlabeled data, which is then added to the training set for a new round of training before classifying remaining sets of data. 
The main difference from the Yarowsky algorithm and our approach is that, rather than using a fully automated process for increasing training data, we use a probability threshold to regulate recall, followed by human judgment to ensure high precision. % evaluators to verify these labels before adding them to the training set. 

% which uses a high precision, low recall Named Entity Recognition (NER) model trained on a small amount of high-quality labelled data to augment a dataset of biomedical entities with data weakly labelled by the NER model. The main difference is that we validate the weakly labelled data before adding it to our dataset and iteratively improving our classifier to gain more confidence in the augmented data. 
 
 Apart from \newcite{clark1989contributing} there have been other taxonomies of grounding. For example, \newcite{traum1999computational} considers six categories; among these are \textit{acknowledge} and \textit{continue}, which, taken together, map nicely to \ya. \newcite{magerkoemp} and \newcite{sharedmental} note the importance of establishing common ground in improv. 
